"If You're Not Doing It, Somebody Else Is": Active Negotiation and the Invisible Labor of Sustained LLM Use

Large language models (LLMs) have become fixtures of academic work even as their users describe them as degrading their writing, thinking, and skills. Dominant adoption frameworks read continued use as evidence of satisfaction, and cannot explain continued use of a distrusted tool. We interviewed 36 graduate student workers, balanced between English-as-a-foreign-language (EFL) and non-EFL speakers, and introduce the Active Negotiation framework: a model of sustained LLM use as a recurring cycle of risk, mitigation, and justification. A failure surfaces a risk, mitigation labor addresses it, and a justification renders the residual risk tolerable until the next failure reopens the cycle. The cycle runs across three dimensions: practical, auditing output; internal, auditing one's own cognition and identity; and social, managing how peers and institutions perceive use. EFL participants invoke linguistic parity as a further justification. We reframe continued adoption as compliance sustained by invisible labor.

==> tables/table_demographics.tex <==
% Table 1: Participant demographics
% Column order matches Tables 2-4 (EFL, Non-EFL, Total).
\begin{table}[htbp]
\centering
\caption{Participant demographics (N=36). Participants were categorized into broad fields of study to protect anonymity.}
\label{tab:demographics}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{l c c c}
\toprule
\textbf{Field of Study} & \textbf{EFL} & \textbf{Non-EFL} & \textbf{Total} \\
 & \textit{(N=15)} & \textit{(N=21)} & \textit{(N=36)} \\
\midrule
STEM     &  9 & 15 & 24 \\
Non-STEM &  6 &  6 & 12 \\
\bottomrule
\end{tabular}

\smallskip
{\footnotesize \textit{Note: EFL participants represented diverse linguistic backgrounds.}}
\end{table}

